Variability-Driven User-Story Generation using LLM and Triadic Concept Analysis

A widely used Agile practice for requirements is to produce a set of user stories (also called ``agile product backlog''), which roughly includes a list of pairs (role, feature), where the role handles the feature for a certain purpose. In the context of Software Product Lines, the requirements for a family of similar systems is thus a family of user-story sets, one per system, leading to a 3-dimensional dataset composed of sets of triples (system, role, feature). In this paper, we combine Triadic Concept Analysis (TCA) and Large Language Model (LLM) prompting to suggest the user-story set required to develop a new system relying on the variability logic of an existing system family. This process consists in 1) computing 3-dimensional variability expressed as a set of TCA implications, 2) providing the designer with intelligible design options, 3) capturing the designer's selection of options, 4) proposing a first user-story set corresponding to this selection, 5) consolidating its validity according to the implications identified in step 1, while completing it if necessary, and 6) leveraging LLM to have a more comprehensive website. This process is evaluated with a dataset comprising the user-story sets of 67 similar-purpose websites.

==> tables/designoptionsanalysis.tex <==
\begin{table}[htb]
\centering
\caption{}
\label{table:designoptionsanalysis}
\adjustbox{width=\linewidth}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
%
\end{tabular}
}%adjustbox
\end{table}

==> tables/tablesmall.tex <==
\begin{table*}[htb]
\centering
\caption{Sets of user-stories from a family of four websites (\texttt{MyManga}, \texttt{MangaStore}, \texttt{MangaFan}, and \texttt{MangaHome}), from \cite{DBLP:journals/ijar/BazinGHMT24}.}
\label{table:us}
\adjustbox{width=0.7\textwidth}{
\begin{tabular}{|c|c|c|}
\hline  
\textbf{Website}&\textbf{Role}&\textbf{Feature}\\
\hline  \hline  
MyManga&user&search\\
\hline  
MyManga&user&viewComment\\
\hline  
MyManga&user&addComment\\
\hline 
MyManga&productOwner&CRUDproducts\\
\hline 
MyManga&communityManager&moderateComment\\
\hline
MangaFan&user&search\\\hline 
MangaFan&user&manageCart\\\hline 
MangaFan&user&pay\\\hline 
MangaFan&user&signUp\\\hline 
MangaFan&admin&CRUDproducts\\\hline 
MangaFan&admin&manageUserAccount\\\hline 
MangaFan&registeredUser&manageProfile\\\hline 
MangaFan&admin&manageProfile\\
\hline \hline
\end{tabular}
\begin{tabular}{|c|c|c|}
\hline  
\textbf{System}&\textbf{Role}&\textbf{Feature}\\
\hline  \hline  
MangaStore&user&search\\
\hline 
MangaStore&user&manageCart\\
\hline 
MangaStore&user&pay\\\hline 
MangaStore&productOwner&makePromotionalCampaign\\\hline 
MangaStore&productOwner&CRUDproducts\\
\hline \hline
MangaHome&user&search\\\hline 
MangaHome&user&viewComment\\\hline 
MangaHome&user&addComment\\\hline 
MangaHome&communityManager&moderateComment\\\hline 
MangaHome&user&signUp\\\hline 
MangaHome&admin&CRUDproducts\\\hline 
MangaHome&admin&manageUserAccount\\\hline 
MangaHome&registeredUser&manageProfile\\\hline 
MangaHome&admin&manageProfile\\\hline 
\end{tabular}
 }
\end{table*}
